Future-conditioned Unsupervised Pretraining for Decision Transformer

Recent research in offline reinforcement learning (RL) has demonstrated that return-conditioned supervised learning is a powerful paradigm for decision-making problems. While promising, return conditioning is limited to training data labeled with rewards and therefore faces challenges in learning from unsupervised data. In this work, we aim to utilize generalized future conditioning to enable efficient unsupervised pretraining from reward-free and sub-optimal offline data. We propose Pretrained Decision Transformer (PDT), a conceptually simple approach for unsupervised RL pretraining. PDT leverages future trajectory information as a privileged context to predict actions during training. The ability to make decisions based on both present and future factors enhances PDT's capability for generalization. Besides, this feature can be easily incorporated into a return-conditioned framework for online finetuning, by assigning return values to possible futures and sampling future embeddings based on their respective values. Empirically, PDT outperforms or performs on par with its supervised pretraining counterpart, especially when dealing with sub-optimal data. Further analysis reveals that PDT can extract diverse behaviors from offline data and controllably sample high-return behaviors by online finetuning. Code is available at here.

==> fig/ablation/context/context.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{fig/ablation/context/evalcontext.pdf}
    \caption{Comparison of finetuning performance on Gym MuJoCo
tasks, when {\ours} is evaluated with different context length. We report the averaged normalized return over 3 random seeds. The error bar shows the
95\% confidence interval.}
    \label{fig:evalcontext}
\end{figure}



==> sec/technique.tex <==
\section{Useful Notes}

\begin{enumerate}
    \item Value function
    \begin{equation*}
        Q^\pi\left(s_t, a_t\right)=\frac{1}{1-\gamma} \mathbb{E}_{s, a \sim \mathbb{P}_{t: H}^\pi\left(s_t, a_t\right), \pi(s)}[r(s, a)],
    \end{equation*}
    where $\mathbb{P}_{t: H}^\pi\left(s \mid s_t, a_t\right)=(1-\gamma) \sum_{\Delta t=1}^H \gamma^{\Delta t-1} \mathbb{P}\left[S_{t+\Delta t}=s \mid s_t, a_t ; \pi\right]$.
    This tells us that ``to estimate
a quantity akin to $Q$, we can first estimate the occupancy measure and take a weighted average of rewards over future states using the probabilities from the log-density ratio learned by the contrastive model''.
    \item Successor representation and successor features

    Successor representation
    \begin{equation*}
        \begin{aligned}
        V^\pi & =\mathbf{r}+\gamma P^\pi \mathbf{r}+\left(\gamma P^\pi\right)^2 \mathbf{r}+\cdots \\
        & =\left(I-\gamma P^\pi\right)^{-1} \mathbf{r} \\
        & =\Lambda^\pi \mathbf{r}
        \end{aligned}
    \end{equation*}

    Successor features (SFs) (Barreto et al., 2017) have been proposed as a generalization to the successor representation. SFs assume that the reward function can be decomposed into a linear combination of features, $r\left(s, a, s^{\prime}\right)=\phi\left(s, a, s^{\prime}\right)^T \mathbf{w}$, where $\phi\left(s, a, s^{\prime}\right)^T$ is a row vector of features and $\mathbf{w}$ is the weights, changing the representation from one based on state visitation to one based on feature occurrences. Using this assumption, successor features $\psi^\pi(s, a)$ are derived from the action-value function for a given policy $\pi, Q^\pi(s, a)$, which we can write as the expected sum of discounted rewards starting from timestep $t$. Here, $r_t$ represents the reward received, while $S_t$ and $A_t$ are random variables representing the state and action taken at $t$, respectively.
    $$
    \begin{aligned}
    Q^\pi(s, a) & =E^\pi\left[\sum_{i=t}^{\infty} \gamma^{i-t} r_{i+1} \mid S_t=s, A_t=a\right] \\
    & =E^\pi\left[\sum_{i=t}^{\infty} \gamma^{i-t} \phi_{i+1}^T \mathbf{w} \mid S_t=s, A_t=a\right] \\
    & =\psi^\pi(s, a)^T \mathbf{w}
    \end{aligned}
    $$
    
    In the tabular case, i.e., where the reward features $\phi\left(s, a, s^{\prime}\right)$ are a one-hot vector in $\mathbb{R}^{|S|^2|A|}$, the SFs become the discounted sum of transition occurrences, thus extending the SR concept from state space to state-action-next-state space. The reward weights $\mathbf{w}$ can also be factored out from the Bellman equation for the action-value function in order to define a new Bellman equation where the reward features take the place of the rewards themselves. This allows us to apply any RL method to learn the SFs. Where $\phi(s, a)=E\left[\phi\left(s, a, s^{\prime}\right)\right]$, this equation is:
    $$
    \psi^\pi(s, a)=\phi(s, a)+\gamma \sum_{s^{\prime}} P\left(s, a, s^{\prime}\right) \psi^\pi\left(s^{\prime}, \pi\left(s^{\prime}\right)\right)
    $$
\end{enumerate}
